Probing the Higgs Boson via VBF with Single Jet Tagging at the LHC

The signature produced by the Standard Model Higgs boson in the Vector Boson Fusion (VBF) mechanism is usually pinpointed by requiring two well separated hadronic jets, one of which (at least) of them tends to be in the forward direction. With the increase of instantaneous luminosity at the LHC, the isolation of the Higgs boson produced with the VBF mechanism is rendered more challenging. In this paper the feasibility of single jet tagging is explored in a high-luminosity scenario. It is demonstrated that the separation in rapidity between the tagging jet and the Higgs boson can be effectively used to isolate the VBF signal. This variable is robust from the experimental and QCD stand points. Single jet tagging allows us to probe the spin-CP quantum numbers of the Higgs boson.

==> Figures/mc_samples.tex <==
\newcommand{\progname}[1]{\textsc{#1}}
% MC generators
\newcommand{\pythiaEight}{\progname{Pythia8}}
\newcommand{\powheg}{\progname{Powheg}}


%%%%%%%%%%%%
%% POWHEG %% 
%%%%%%%%%%%%
For this paper, events were privately generated for the two production modes: gluon-gluon fusion and vector boson fusion.  
The gluon-gluon fusion events were generated using the \progname{Powheg} HJJ process~\cite{Campbell:2012am}, and are accurate to NLO for Higgs produced in association with up to two jets.
HJJ was used in association with MINLO (Multi-scale improved NLO)~\cite{MINLO,Hamilton:2012np}, 
%which uses the CKKW prescription~\cite{Catani:2001cc,Krauss:2002up,Mrenna:2003if}
which sets the emission scales to the $p_T$ of the emitted partons. 
The VBF events were also produced with \progname{Powheg}~\cite{powheg_VBF} and are also accurate at NLO.
Both samples were produced for a Higgs mass of 126.8 GeV and using the CT10 parton distribution function~\cite{PDF:CT10}.

%%%%%%%%%%%%
%% PYTHIA %%
%%%%%%%%%%%%
The samples were then interfaced with \progname{Pythia8}~\cite{pythia8},	
which adds the showering and hadronization of the events as well as the underlying event.
Within Pythia, stable particles are clustered into jets using the anti-$k_\mathrm{t}$ algorithm~\cite{JetAlgo} with a cone size of $\Delta R=0.4$

%%%%%%%%%%%%%%%%%%%
%% FIDUCIAL CUTS %%
%%%%%%%%%%%%%%%%%%%
The following fiducial cuts were applied to the samples.  The $p_T$ of the leading (subleading) photon is required to be greater than 40 (30) GeV and within a rapidity $\left|y\right|<2.4$.  In addition, the photons are isolated, which is accomplished by requiring the amount of transverse energy within $\Delta R=0.4$ to be less than 14 GeV.  Jets are then required to have $p_T>30\,$GeV and to be within a rapidity $\left|y\right|<4.4$. An overlap removal is applied on jets, where any jet within $\Delta R<0.4$ of a photon is removed, and any jet within $\Delta R<0.2$ of an electron is removed.
% electrons are also isolated and have pT>15 GeV and |y|<2.47


%%%%%%%%%%%%%%%%%%%%
%% VBF 2-JET CUTS %%
%%%%%%%%%%%%%%%%%%%%
Events with more than one jet were then classified as VBF-like, which is defined by the following:
\begin{itemize}
 \item $\Delta\eta_{jj} >$ 2.8
 \item $M_{jj} >$ 520 GeV
 \item $\eta_{H}-\frac{\eta_{j1}+\eta_{j2}}{2} <$ 2.4
 \item $\Delta\phi_{H,jj} >$ 2.6
\end{itemize}





==> Figures/table_VBF_1jet-1.tex <==

\begin{table}[htbp]\tiny
  \begin{tabular}{cccccccccccc}

  \hline
  pT Cut & $\Delta\eta$ Cut & Signal & Bkg & S/B & $\Delta\mu$ & Signal & Bkg & S/B & $\Delta\mu$ & Total $\Delta\mu$ \\
  \hline
30 & 1.40 & 137.321 & 30.668 & 4.478 & 0.095 & 261.526 & 1203.739 & 0.217 & 0.146 & 0.080
35 & 1.40 & 120.202 & 25.320 & 4.747 & 0.101 & 255.874 & 988.994 & 0.259 & 0.138 & 0.081
40 & 1.40 & 103.333 & 20.985 & 4.924 & 0.108 & 247.336 & 814.661 & 0.304 & 0.132 & 0.084
45 & 1.40 & 87.569 & 17.285 & 5.066 & 0.117 & 235.912 & 681.020 & 0.346 & 0.128 & 0.087
50 & 1.40 & 73.577 & 14.827 & 4.962 & 0.128 & 222.203 & 573.959 & 0.387 & 0.127 & 0.090
55 & 1.40 & 61.162 & 12.139 & 5.039 & 0.140 & 207.925 & 482.780 & 0.431 & 0.126 & 0.094
  \hline

  \end{tabular}
\end{table}



==> Figures/table_VBF_1jet-2.tex <==

\begin{table}[htbp]\tiny
  \begin{tabular}{cccccccccccc}

  \hline
%  pT Cut & $\Delta\eta$ Cut & Signal & Bkg & S/B & $\Delta\mu$ & Signal & Bkg & S/B & $\Delta\mu$ & Total $\Delta\mu$ \\
  pT Cut & $\Delta y$ Cut & Signal & Bkg & S/B & $\Delta\mu$ & Signal & Bkg & S/B & $\Delta\mu$ & Total $\Delta\mu$ \\
  \hline

%%%%%%%%%%%%%%%%
\begin{comment}
30 & 1.40 & 137.321 & 30.668 & 4.478 & 0.095 & 261.526 & 1203.739 & 0.217 & 0.146 & 0.080
35 & 1.40 & 120.202 & 25.320 & 4.747 & 0.101 & 255.874 & 988.994 & 0.259 & 0.138 & 0.081
40 & 1.40 & 103.333 & 20.985 & 4.924 & 0.108 & 247.336 & 814.661 & 0.304 & 0.132 & 0.084
45 & 1.40 & 87.569 & 17.285 & 5.066 & 0.117 & 235.912 & 681.020 & 0.346 & 0.128 & 0.087
50 & 1.40 & 73.577 & 14.827 & 4.962 & 0.128 & 222.203 & 573.959 & 0.387 & 0.127 & 0.090
55 & 1.40 & 61.162 & 12.139 & 5.039 & 0.140 & 207.925 & 482.780 & 0.431 & 0.126 & 0.094
\end{comment}
%%%%%%%%%%%%%%%%

30 & 1.30 & 137.321 & 30.668 & 4.478 & 0.095 & 286.643 & 1174.725 & 0.244 & 0.133 & 0.077 \\
35 & 1.30 & 120.202 & 25.320 & 4.747 & 0.101 & 279.768 & 972.120 & 0.288 & 0.126 & 0.079  \\
40 & 1.30 & 103.333 & 20.985 & 4.924 & 0.108 & 269.527 & 807.733 & 0.334 & 0.122 & 0.081  \\
45 & 1.30 & 87.569 & 17.285 & 5.066 & 0.117 & 256.496 & 676.954 & 0.379 & 0.119 & 0.084   \\
50 & 1.30 & 73.577 & 14.827 & 4.962 & 0.128 & 240.962 & 573.912 & 0.420 & 0.118 & 0.087   \\
55 & 1.30 & 61.162 & 12.139 & 5.039 & 0.140 & 224.888 & 485.647 & 0.463 & 0.119 & 0.091   \\

  \hline

  \end{tabular}
\end{table}



==> Figures/table_VBF_1jet.tex <==

\begin{table}[htbp]\tiny
  \begin{tabular}{cccccccccccc}

  \hline
  pT Cut & $\Delta\eta$ Cut & Signal & Bkg & S/B & $\Delta\mu$ & Signal & Bkg & S/B & $\Delta\mu$ & Total $\Delta\mu$ \\
  \hline
  30 & 1.40 & 137.32 & 30.67 & 4.48 & 0.10 & 261.53 & 1203.74 & 0.22 & 0.15 & 0.08
  35 & 1.40 & 120.20 & 25.32 & 4.75 & 0.10 & 255.87 & 988.99 & 0.26 & 0.14 & 0.08
  40 & 1.40 & 103.33 & 20.98 & 4.92 & 0.11 & 247.34 & 814.66 & 0.30 & 0.13 & 0.08
  45 & 1.40 & 87.57 & 17.29 & 5.07 & 0.12 & 235.91 & 681.02 & 0.35 & 0.13 & 0.09
  50 & 1.40 & 73.58 & 14.83 & 4.96 & 0.13 & 222.20 & 573.96 & 0.39 & 0.13 & 0.09
  55 & 1.40 & 61.16 & 12.14 & 5.04 & 0.14 & 207.92 & 482.78 & 0.43 & 0.13 & 0.09
  \hline

  \end{tabular}
\end{table}


